No domain left behind: is Let's Encrypt democratizing encryption?

The 2013 National Security Agency revelations of pervasive monitoring have lead to an "encryption rush" across the computer and Internet industry. To push back against massive surveillance and protect users privacy, vendors, hosting and cloud providers have widely deployed encryption on their hardware, communication links, and applications. As a consequence, the most of web traffic nowadays is encrypted. However, there is still a significant part of Internet traffic that is not encrypted. It has been argued that both costs and complexity associated with obtaining and deploying X.509 certificates are major barriers for widespread encryption, since these certificates are required to established encrypted connections. To address these issues, the Electronic Frontier Foundation, Mozilla Foundation, and the University of Michigan have set up Let's Encrypt (LE), a certificate authority that provides both free X.509 certificates and software that automates the deployment of these certificates. In this paper, we investigate if LE has been successful in democratizing encryption: we analyze certificate issuance in the first year of LE and show from various perspectives that LE adoption has an upward trend and it is in fact being successful in covering the lower-cost end of the hosting market.

==> 08-discussion.tex <==
public suffix vs. 2LD

\iftoggle{thesis}{%
(TODO, rewrite) We will now examine \LE's contribution based on the barriers described in the previous section.
Certificate cost is zero and unlikely to raise any time soon given ISRG's mission and the lack of support for billing in ACME. This is therefore a monetary differentiator against a part of the market, representing the removal of a significant barrier. Deployment cost naturally remains. However, with the repeated certificate request, issuance and installation are replaced by a one-time installation/configuration of an ACME client, the certificate renewal cost is cut\footnote{ACME clients being software, there is a recurring cost of updating and patching, yet these costs are amortized over all domains.}. This is a differentiator versus the bulk of the CA market, representing the removal of a significant recurring investment barrier\footnote{The author are not familiar with the average lifetime of (vanity) domains in the shared hosting segment. If these are shorter than the average period of certificate issuance, then our claim only partly holds.}. In the third category of complexity cost, \LE, by virtue of its support for automating renewal by means of ACME clients reduces the chance of service downtime due to forgotten certificate renewal. % Finally, one may argue that some ACME clients are especially tailored to reduce human configuration effort. We counter that the typical shared hosting environment may be harder to autoconfigure than the stock configurations they target, which is why we don't list this as a significant differentiator.
% Last, with reference to the ``standard service offering'' incentive described earlier, we note that a number of software solution for the management of shared web hosting environments (Plesk, cPanel) are including support for ACME. If these were ever be turned into default configuration, use of \LE may become a non-conscious decision on the part of shared hosting providers.
}{}

